Single Day Outdoor Photometric Stereo

Photometric Stereo (PS) under outdoor illumination remains a challenging, ill-posed problem due to insufficient variability in illumination. Months-long capture sessions are typically used in this setup, with little success on shorter, single-day time intervals. In this paper, we investigate the solution of outdoor PS over a single day, under different weather conditions. First, we investigate the relationship between weather and surface reconstructability in order to understand when natural lighting allows existing PS algorithms to work. Our analysis reveals that partially cloudy days improve the conditioning of the outdoor PS problem while sunny days do not allow the unambiguous recovery of surface normals from photometric cues alone. We demonstrate that calibrated PS algorithms can thus be employed to reconstruct Lambertian surfaces accurately under partially cloudy days. Second, we solve the ambiguity arising in clear days by combining photometric cues with prior knowledge on material properties, local surface geometry and the natural variations in outdoor lighting through a CNN-based, weakly-calibrated PS technique. Given a sequence of outdoor images captured during a single sunny day, our method robustly estimates the scene surface normals with unprecedented quality for the considered scenario. Our approach does not require precise geolocation and significantly outperforms several state-of-the-art methods on images with real lighting, showing that our CNN can combine efficiently learned priors and photometric cues available during a single sunny day.

==> hdr-database.tex <==
%\section{Outdoor lighting conditions analysis}

%To explore the richness of natural illumination in the context of Photometric Stereo (PS), we exploit the database of outdoor HDR environment maps detailed in the last section, which provides a rich sampling of the variability of outdoor illumination. To ensure the data is properly aligned temporally, only images that were captured during a continuous 6 hour time interval on each of these days, from 10{:}30 until 16{:}30, are considered. Through a theoretical analysis (inspired by \cite{sun-ivc-07}) and supported by an extensive empirical evaluation as well as a preliminary quantitative validation, we derive confidence intervals that allow us to predict when surface normals can be reconstructed more accurately and solely from the photometric cue. Instead of focusing exclusively on sun position~\cite{shen-pg-14}, our analysis incorporates the influence of all components of natural lighting: sun, sky, clouds, etc., as well as noise and surface albedo. 

\section{HDR database}
\label{sec:hdrdb}

So far, in most literature on Photometric Stereo, the light visible by a surface patch is modeled with simple directional illumination, where optimal lighting configurations can be theoretically derived~\cite{drbohlav-iccv-05,klaudiny-prl-14,shen-pg-14}. Until recently, no attempt has been made yet to model natural lighting conditions with more realistic illumination models in an outdoor setup, where lighting cannot be controlled and atmospheric effects are difficult to predict. In such an uncontrolled environment, exploiting the subtlety and richness of natural lighting is key to increase the efficiency of PS and successfully apply it to short intervals of time in the wild.

In order to understand this complex natural phenomenon, we use HDRDB~\cite{hdrdb}, a rich dataset of High Dynamic Range (HDR) images of the sky, captured under a wide variety of conditions. In all, the dataset totals more than 5,000 illumination conditions, captured over 50 different days. Fig.~\ref{fig:database} shows examples of these environment maps, which are tone mapped for display only; the actual sky images have extremely high dynamic range, and span the full 22 stops required to properly capture outdoor lighting. %, as shown in fig.~\ref{fig:exposure}.

%To build this database, we captured HDR images of the sky hemisphere using the approach described in \cite{stumpfel-afrigraph-04}. Pictures of the capture system are shown in fig.~\ref{fig:capture-apparatus}. For each image, we captured seven exposures of the sky ranging from 1/8000 to 1 second, using a Canon EOS 5D Mark III camera installed on a tripod, and fitted with a SIGMA EXDG 8mm fisheye lens. A 3.0 ND filter was installed behind the lens, necessary to accurately measure the sun intensity. The exposures were stored as 14-bit RAW images at the full resolution of the camera. The camera was controlled using a Raspberry Pi via a USB connection, and the setup was mounted on the roof of a tall building to capture the entire sky hemisphere. Every two minutes, we captured the seven exposures required to span the full dynamic range of the outdoor sky. The fisheye lens was radiometrically calibrated to account for chromaticity shifts caused by the ND filter, geometrically calibrated using~\cite{scaramuzza-iros-06}, and the resulting light probes mapped to the angular environment map representation~\cite{reinhard-book-05} for storage in floating-point EXR format. We merged the seven exposures using~\cite{debevec-siggraph-97} to create one HDR sky probe per exposure set.

%Because the camera may have shifted from one capture day to another, we automatically align all sky probes to the world reference frame. This was done by detecting the sun in at least 3 images for a given day, and by computing the rotation matrix which best aligned the detected positions and the real sun coordinates (obtained with~\cite{reda-se-04}). For days when the sun was never visible, the probes were manually aligned using other aligned light probes as examples, and by matching visible buildings close to the horizon.



%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{exposureFig/exposureFig-row.pdf}
%\includegraphics[width=0.9\linewidth]{exposureFig/exposureFig-row.jpg}
%\caption[Sky Database]{Dynamic range in our sky database. Four different exposures of the same sky probe are shown, each expressed as factors (indicated as insets) of a reference image (1). The left-most image appears completely black, but zooming in (inset) reveals that the sun intensity is captured without saturation.}
%\label{fig:exposure}
%\end{figure}


%\begin{figure}
%\centering
%\includegraphics[width=0.45\linewidth]{database/capture_apparatus.jpg}
%\includegraphics[width=0.45\linewidth]{database/capture_apparatus_inside.jpg}
%\caption[Database capture apparatus]{Left: sky capture apparatus we developed. Right: the inside of the box, holding the Canon 5D mark III and the Raspberry Pi control system.}
%\label{fig:capture-apparatus}
%\end{figure}


%In the rest of this chapter, we explore the conditions in which PS may or may not work, when faced with the challenging case of uncontrollable outdoor illumination. 

% Or, in other words: what makes it a good day for outdoor Photometric Stereo? 

%As one might expect, the answer to the question above is intrinsically tied to the orientation of a particular surface patch, the associated hemisphere of lighting directions observed by the patch, and the variation in lighting intensity in that hemisphere over the course of a day. So far, this question has only been explored in laboratory conditions or with simple directional illumination, where optimal lighting configurations can be theoretically derived~\cite{drbohlav-iccv-05,klaudiny-prl-14,shen-pg-14}. No attempt has been made at answering this question with more realistic illumination models in an outdoor setup, where lighting cannot be controlled and atmospheric effects are difficult to predict.


